CARL-GT: Evaluating Causal Reasoning Capabilities of Large Language Models

Causal reasoning capabilities are essential for large language models (LLMs) in a wide range of applications, such as education and healthcare. But there is still a lack of benchmarks for a better understanding of such capabilities. Current LLM benchmarks are mainly based on conversational tasks, academic math tests, and coding tests. Such benchmarks evaluate LLMs in well-regularized settings, but they are limited in assessing the skills and abilities to solve real-world problems. In this work, we provide a benchmark, named by CARL-GT, which evaluates CAusal Reasoning capabilities of large Language models using Graphs and Tabular data. The benchmark has a diverse range of tasks for evaluating LLMs from causal graph reasoning, knowledge discovery, and decision-making aspects. In addition, effective zero-shot learning prompts are developed for the tasks. In our experiments, we leverage the benchmark for evaluating open-source LLMs and provide a detailed comparison of LLMs for causal reasoning abilities. We found that LLMs are still weak in casual reasoning, especially with tabular data to discover new insights. Furthermore, we investigate and discuss the relationships of different benchmark tasks by analyzing the performance of LLMs. The experimental results show that LLMs have different strength over different tasks and that their performance on tasks in different categories, i.e., causal graph reasoning, knowledge discovery, and decision-making, shows stronger correlation than tasks in the same category.

==> tables/cdir.tex <==
\begin{table}[h]
    \centering     
    \caption{Benchmark on tables with causal direction estimation. $10$ causal graphs. 
    The unknown answers that are replaced by random yes or no.
    Gemma cannot only take 20 rows of tables as inputs, while the others take 50 rows. The answers are limited by yes or no.}\label{tab:causal_table_cdir}
    \begin{tabular}{c|c}
    \hline
	  	 & MAE 	 \\ \hline
Llama3 7B &$0.321$\\
Qwen2 7B &$0.00$ \\
Mistral 7B &$0.429$\\
Gemma 9B &$0.00$ \\
Mistral 8x7B &$0.00$\\
\hline
\end{tabular}
\end{table}


==> tables/cf.tex <==
\begin{table}[h]
    \centering     
    \caption{Benchmark on the interventional and counterfactual inference tasks. The answers with unknown responses are skipped. Gemma only take 20s rows of tables as inputs and failed to reply to the question, while the others are prompted by tables with 50 rows and corresponding causal graphs. }\label{tab:ci_cf}
    \begin{tabular}{c|c}
    \hline
	  	 & CF-AUC 	 \\ \hline
Llama3 7B &$1.586 \pm 1.060$\\
Qwen2 7B & $1.475 \pm 0.642$ \\
Mistral 7B &$1.500 \pm 0.661$\\
Gemma 9B &$-$ \\
Mistral 8x7B &$1.125 \pm 0.359$\\
\hline
\end{tabular}
\end{table}


==> tables/ci_50_nodes.tex <==
\begin{table}
    \centering     
    \caption{Benchmark on the interventional and counterfactual inference tasks. The answers with unknown responses are skipped. LLMs are prompted with $10$ causal graphs and corresponding tables with 50 rows. }\label{tab:ci}
    \begin{tabular}{c|cc}
    \hline
	  	 & inv-MAE $\downarrow$ 	  & cf-MAE $\downarrow$ 	 \\ \hline
Llama3&$9.071 \pm 8.793$ & $8.572 \pm 6.770$\\
Qwen2-20r  & $2.449 \pm 1.344$&$0.971 \pm 0.393$  \\
Mistral  &$1.645 \pm 0.832$& $5.003 \pm 2.102$\\
% Gemma  &$-$ &$-$ \\
% Mixtral &$2.409 \pm 1.407$&$\mathbf{1.125 \pm 0.359}$\\
\hline
\end{tabular}
   
\end{table}


==> tables/citable.tex <==
\begin{table}[h]
    \centering     
    \caption{Benchmark on tables with d-seperation estimation. $10$ causal graphs. The unknown answers that are replaced by random yes or no. Gemma cannot only take 20 rows of tables as inputs, while the others take 50 rows. The answers are limited by yes or no.}\label{tab:causal_table_ci}
    \begin{tabular}{c|c}
    \hline
	  	 & tab-AUC 	 \\ \hline
Llama3 7B &$0.562$\\
Qwen2 7B &$0.50$ \\
Mistral 7B &$0.554$\\
Gemma 9B &$0.50$ \\
Mistral 8x7B &$-$\\
\hline
\end{tabular}
\end{table}


==> tables/com_gen_dis.tex <==
\begin{table}[h]
    \centering     
    \caption{Comparision of applying LLMs to causal inference and discovery tasks in a generative and  discriminative way. The LLMs are evaluated on $5$ causal graphs and their corresponding tables. Tables with $100$ rows used in the question prompts. The generative way first asks LLMs to generate synthetic tabular data and then applies different causal discovery and causal inference methods to get the final answers based on the synthetic data. References are the results by using benchmark data.}\label{tab:comp}
\begin{tabular}{c|cccc}
    \hline
	  	 & intv-MAE $\downarrow$	& cf-MAE $\downarrow$	 & AUC $\uparrow$	  & Acc. 	$\uparrow$ \\ \hline
Qwen2 & $2.281 \pm 0.640$ & $2.001 \pm 0.913$ & $0.50$  & $0$ \\
Mistral &$1.908 \pm 0.760$&$2.732 \pm 2.228$&$0.542$&$0.449$\\\hline
Qwen2-Gen &$0.557 \pm 0.484$ &$0.056 \pm 0.106$ &$0.757$&$0.724$ \\
Mistral-Gen &$0.428 \pm 0.623$&$0.047 \pm 0.058$&$0.609 $&$0.621$\\\hline
ref-Gen & $0.057 \pm 0.021$ & $0.00076 \pm 0.0014$ & $0.882$ & $0.966$ \\
\hline
\end{tabular}
\end{table}


==> tables/graph_50_nodes.tex <==
\begin{table}
    \centering     
    \caption{Benchmark on causal graph reasoning.
    As for adjacency matrix estimation, LLMs are required to recover $10$ causal graphs for with bootstrapping $5$ times. The metrics are F1 scores, recall, and precision. As for d-separation estimation, LLMs classify d-separated and d-connected relationships chosen from $10$ causal graphs. And the metric is the AUC of ROC curves.}\label{tab:causal_graph}
    \begin{tabular}{c|ccc|c|ccc}
    \hline
	  	 & f1 $\uparrow$ 	 & precision $\uparrow$ 	& recall $\uparrow$  & AUC $\uparrow$ & f1 $\uparrow$ 	 & precision $\uparrow$ 	& recall $\uparrow$  	  	\\\hline
Llama3 &$0.46\pm0.06$ &$0.31\pm0.05$ &$ 0.98\pm0.02$& running&$0.46\pm0.22$ &$0.36\pm0.18$ &$ 0.66\pm0.30$\\
Qwen2 &$0.39\pm0.08$ &$0.25\pm0.06$ &$ 0.91\pm0.05$& running &$0.09\pm0.06$ &$0.11\pm0.10$ &$ 0.17\pm0.20$\\
Mistral &$0.34\pm0.11$ &$0.24\pm0.08$ &$ 0.63\pm0.30$&  $0.493$&$0.52\pm0.18$ &$0.47\pm0.10$ &$ 0.62\pm0.23$\\
% Gemma2  &$0.81\pm0.16$ &$0.71\pm0.24$ &$\mathbf{1.00\pm0.00}$&$\mathbf{0.562}$&&&\\
% Mixtral  &$\mathbf{0.95\pm0.04}$ &$\mathbf{1.00\pm0.00}$ &$ 0.92\pm0.07$&$0.482$&&&\\
\hline
\end{tabular}
\end{table}


==> tables/tab.tex <==

\begin{table}[h!]
\centering
\caption{Benchmark tabular synthesis ability of LLMs from the perspectives of causality. The input prompts are based on tables with $100$ rows and the synthetic datasets generated by LLMs have $400$ samples for each causal graph. The evaluation is based the benchmark of \citep{tu24}.} \label{tab:llm}
\begin{tabular}{c|ccc|cc}
\hline
Model  & adj-F1$\uparrow$ & ci-AUC $\uparrow$  & cdir-Acc. $\uparrow$  & intv-MAE $\downarrow$ & cf-MAE $\downarrow$  \\
\hline
real&  $0.79\pm 0.07$&$0.868$& $1.0$ & $0.004 \pm 0.002$ & $0.0004 \pm 0.001$\\
\hline
Qwen2& $0.55\pm 0.09$&$0.757$&$0.724$&$0.283 \pm 0.315$& $0.008 \pm 0.009$\\
% Qwen-200i& $0.67\pm 0.13$&$0.725$&$0.897$&$0.00969 \pm 0.0022$& $0.0023 \pm 0.0012$\\
Mixtral&$0.42\pm 0.09$&$0.609$&$0.621$&$0.661 \pm 0.959$&$0.141 \pm 0.008$\\
% \hline
% \makecell{LLAMA-3 \\(8B-instruct)} &-&-&-&-&-&-&-&-&-\\
% Gemma2&-&-&-&-&-&-&-&-&-\\
% \hline
% ChatGPT&dd&dd&&&&&\\
% GPT-4&dd &dd &&&&&\\
% Claude-3 &dd&dd&&&&&\\
% Gemini-nano&dd&dd&&&&&\\
\hline
\end{tabular}
\label{table:simple}
\end{table}

==> tables/table_50_nodes.tex <==
\begin{table}
\centering     
\caption{Benchmark on causal knowledge discovery. As for d-separation and causal direction estimation, the answers are limited by yes or no. The questions are based on $10$ causal graphs. When there are unknown answers from LLMs, we replaced by random yes or no. Gemma only takes no more than 20 rows of tables as inputs, so we input tables with $20$ rows for Gemma while the others take input tables with $50$ rows.
}\label{tab:table}
\begin{tabular}{c|cc}
\hline
	  	  & AUC $\uparrow$ 	 & Acc. $\uparrow$ 	 \\ \hline
Llama3 &$NA$ &$NA$\\
Qwen2-20r  &$0.5$ &$0.0$ \\
Mistral  &running&$0.1724$\\
\hline
\end{tabular}
\end{table}

